Are neighbourhood amenities associated with more walking and less driving? Yes, but only for the wealthy

Cities are home to a vast array of amenities, from local barbers to science museums and shopping malls. But these are inequality distributed across urban space. Using Google Places data combined with trip-based mobility data for Bogot\'a, Colombia, we shed light on the impact of neighbourhood amenities on urban mobility patterns. Deriving a new accessibility metric that explicitly takes into account spatial range, we find that a higher density of local amenities is associated a higher likelihood of walking as well as shorter bus and car trips. Digging deeper, we use a sample stratification framework to show that socioeconomic status (SES) modulates these effects. Amenities within about a 1km radius are strongly associated with a higher propensity to walk and lower driving time only for only the wealthiest group. In contrast, a higher density of amenities is associated with shorter bus trips for low and middle SES residents. As cities globally aim to boost public transport and green travel, these findings enable us to better understand how commercial structure shapes urban mobility in highly income-segregated settings.

==> tables/freq.tex <==

%\begin{figure}
%\setlength{\fboxsep}{0pt}%
%\setlength{\fboxrule}{0pt}%
%\begin{center}
%\begin{boxedverbatim}
\begin{table}

\scriptsize\sf\centering
\caption{Effects of accessibility on trip frequency}
\textbf{Dep. Variables}: Pr($|trips|=k$ for $k=1...|walk\;trips|$) (Poisson regression on respondents);\\ $freq_i$ (WLS on cells) \\
\begin{tabular}{c | c c c c}
\toprule
\textbf{Ind. Variable}  & $respondents$&  & $cells$&  \\ 
\midrule
$CA_i(walk)$  &0.13***&     0.05***   &   0.04***  &  0.01**   \\
               & (0.01)  &   (0.01)   &    (0.01) & (0.01)     \\
$stratum_i$     &       &   0.14***  &         &  0.05***  \\
                &       &   (0.01)    &          &   (0.01)  \\
$Const$       & -1.05***   &   -1.44***    & 0.35*** &   0.20***  \\
             &  (0.01)    &  (0.04)    & (0.01)  &    (0.02)   \\ 
 \midrule
N  &8826& 8826 & 122& 122\\
Pseudo-$R^2$          &0.00  &    0.01            & &\\
$R^2$           &           &          &0.23 &0.30\\
\bottomrule
\end{tabular}
\label{table:freq}
\end{table}
%\end{boxedverbatim}
%\end{center}
%\caption{Example table layout.\label{F2}}
%\end{figure}


==> tables/legacy_walking.tex <==
\\
B. \textbf{Dep. Variable}: Pr($mode_t=walk$) (logistic regression on trips $0-15$ min); \\Pr($|walk \;trips =k$ for $k=1..|walk\;trips\;0-15$ min) (Poisson regression on respondents); \\$\% walking\;trips$ $0-15$ min (WLS on cells) \\

\begin{tabular}{c | c c c c c c }
\toprule
\textbf{Ind. Variable} & $trips$  & & $respondents$&  & $cells$&  \\ 
\midrule
$CA_i(walk)$  &-0.36***&     0.11   &   -0.06**  &  0.03   & -0.05*** &0.02\\
               & (0.07)  &   (0.09)   &    (0.03) & (0.04)      & (0.01)&(0.02)\\
$stratum_i$     &       &   -0.49***  &         &  -0.10***  & & -0.08***\\
                &       &   (0.06)    &          &   (0.03)  &&(0.01)\\
$Const$       & 1.68***   &   2.98***    & -1.23*** &   -0.98***   & 0.84***&1.05***\\
             &  (0.05)    &  (0.18)    & (0.02)  &    (0.03)   & (0.01)&(0.03)\\ 
        
        \midrule
N      (individuals)&3009 &  3009 & 2820& 2280 & 115& 115\\
Pseudo-$R^2$          &0.01  &    0.03      & 0.00  &0.00       & &\\
$R^2$           &           &               &       &           &0.10 &0.34
\bottomrule
\end{tabular}
\\
C. \textbf{Dep. Variable}: Pr($mode_t=walk$) (logistic regression on trips $\ge15$ min); \\Pr($|walk \;trips =k$ for $k=1..|walk\;trips\;\ge15$ min) (Poisson regression on respondents); \\$\% walking\;trips$ $\ge15$ min (WLS on cells) \\

\begin{tabular}{c | c c c c c c }
\toprule
\textbf{Ind. Variable} & $trips$  & & $respondents$&  & $cells$&  \\ 
\midrule
$CA_i(walk)$  &-0.10***&     0.11**   &   -0.08***  &  0.07*   & -0.02 &0.03\\
               & (0.04)  &   (0.05)   &    (0.03) & (0.04)      & (0.01)&(0.02)\\
$stratum_i$     &       &   -0.25***  &         &  -0.18***  & & -0.05***\\
                &       &   (0.04)    &          &   (0.03)  &&(0.01)\\
$Const$       & -0.75***   &   -0.09& -2.18*** &   -1.70***   & 0.32***&0.45***\\
             &  (0.03)    &  (0.10)    & (0.02)  &    (0.09)   & (0.01)&(0.03)\\ 
        
        \midrule
N      (individuals)&6816 &  6816 & 6409& 6409 & 118& 118\\
Pseudo-$R^2$          &0.00 &    0.01      & 0.00  &0.00       & &\\
$R^2$           &           &               &       &           &0.02 &0.16
\bottomrule
\end{tabular}



\\
B. \textbf{Dep. Variable}: Pr($mode_t=walk$) (logistic regression on trips $0-15$ min); \\Pr($|walk \;trips =k$ for $k=1..|walk\;trips\;0-15$ min) (Poisson regression on respondents); \\$\% walking\;trips$ $0-15$ min (WLS on cells) \\

\begin{tabular}{c | c c c c c c }
\toprule
\textbf{Ind. Variable} & $trips$  & & $respondents$&  & $cells$&  \\ 
\midrule
$CA_i(walk)$  &-0.36***&     0.11   &   -0.06**  &  0.03   & -0.05*** &0.02\\
               & (0.07)  &   (0.09)   &    (0.03) & (0.04)      & (0.01)&(0.02)\\
$stratum_i$     &       &   -0.49***  &         &  -0.10***  & & -0.08***\\
                &       &   (0.06)    &          &   (0.03)  &&(0.01)\\
$Const$       & 1.68***   &   2.98***    & -1.23*** &   -0.98***   & 0.84***&1.05***\\
             &  (0.05)    &  (0.18)    & (0.02)  &    (0.03)   & (0.01)&(0.03)\\ 
        
        \midrule
N      (individuals)&3009 &  3009 & 2820& 2280 & 115& 115\\
Pseudo-$R^2$          &0.01  &    0.03      & 0.00  &0.00       & &\\
$R^2$           &           &               &       &           &0.10 &0.34
\bottomrule
\end{tabular}
\\
C. \textbf{Dep. Variable}: Pr($mode_t=walk$) (logistic regression on trips $\ge15$ min); \\Pr($|walk \;trips =k$ for $k=1..|walk\;trips\;\ge15$ min) (Poisson regression on respondents); \\$\% walking\;trips$ $\ge15$ min (WLS on cells) \\

\begin{tabular}{c | c c c c c c }
\toprule
\textbf{Ind. Variable} & $trips$  & & $respondents$&  & $cells$&  \\ 
\midrule
$CA_i(walk)$  &-0.10***&     0.11**   &   -0.08***  &  0.07*   & -0.02 &0.03\\
               & (0.04)  &   (0.05)   &    (0.03) & (0.04)      & (0.01)&(0.02)\\
$stratum_i$     &       &   -0.25***  &         &  -0.18***  & & -0.05***\\
                &       &   (0.04)    &          &   (0.03)  &&(0.01)\\
$Const$       & -0.75***   &   -0.09& -2.18*** &   -1.70***   & 0.32***&0.45***\\
             &  (0.03)    &  (0.10)    & (0.02)  &    (0.09)   & (0.01)&(0.03)\\ 
        
        \midrule
N      (individuals)&6816 &  6816 & 6409& 6409 & 118& 118\\
Pseudo-$R^2$          &0.00 &    0.01      & 0.00  &0.00       & &\\
$R^2$           &           &               &       &           &0.02 &0.16
\bottomrule
\end{tabular}

==> tables/linear_time.tex <==

%\begin{figure}
%\setlength{\fboxsep}{0pt}%
%\setlength{\fboxrule}{0pt}%
\begin{center}
%\begin{boxedverbatim}
\begin{table}

\scriptsize\sf\centering
\caption{Effects of accessibility on trip behavior}
\textbf{Dep. Variable}: $time_{t,u,i}$ (all modes)\\

\begin{tabular}{c | c c c c c c }
\toprule
\textbf{Ind. Variable} & $trips$ &  & $respondents$ & & $cells$ & \\ 
\midrule
$CA_i(poly)$  & -1.4**  &     1.2   &   -1.7**  &  1.0   & -2.4** &0.0\\
               & (0.6)  &   (0.8)   &    (0.7) & (0.8)      & (1.1)&(1.2)\\
$stratum_i$     &       &   -3.8***  &           &  -3.9***  & & -4.2***\\
                &       &   (0.7)    &          &   (0.7)  &&(1.1)\\
$Const$       & 46.9***   &   57.2***    & 48.7*** &   59.3***   & 49.5***&60.4***\\
             &  (0.5)    &  (1.9)    & (0.6)  &    (2.0)   & (0.9)&(3.1)\\ 
        
        \midrule
N      (individuals)&13748 &  13748 &  12286&  12286 & 119 & 119\\
$R^2$          &0.00  &    0.00      & 0.00  &0.00       & 0.04 &0.14\\

\bottomrule
\end{tabular}
\\

\textbf{Dep. Variable}: $time_{t,u,i}$ (walking)\\

\begin{tabular}{c | c c c c c c }
\toprule
\textbf{Ind. Variable} & $trips$ &  & $respondents$ & & $cells$ & \\ 
\midrule
$CA_i(walk)$  & 1.0&     1.0   &   0.9  &  0.8   & -0.5 &-0.9\\
               & (0.7)  &   (1.0)   &    (0.7) & (1.0)      & (0.8)&(1.0)\\
$stratum_i$     &       &   -0.0  &         &  0.0  & & 0.6\\
                &       &   (0.7)    &          &   (0.8)  &&(0.8)\\
$Const$       & 23.8***   &   23.8***    & 24.0*** &   23.8***   & 23.4***&22.0\\
             &  (0.5)    &  (1.9)    & (0.5)  &    (2.0)   & (0.6)&(2.0)\\ 
        
        \midrule
N      (individuals)&6193 &  6193 &  12286&  12286 & 119 & 119\\
$R^2$          &0.00  &    0.00      & 0.00  &0.00       & 0.00 &0.01\\

\bottomrule
\end{tabular}
\\
\textbf{Dep. Variable}: $time_{t,u,i}$ (bike trips)\\

\begin{tabular}{c | c c c c c c }
\toprule
\textbf{Ind. Variable} & $trips$ &  & $respondents$ & & $cells$ & \\ 
\midrule
$CA_i(bike)$  & 13.4**&   20.1***   &   13.5**  & 20.5***   & 11.4 &20.1**\\
               & (6.0)  &   (7.2)   &    (6.3) & (7.7)      & (7.5)&(9.0)\\
$stratum_i$     &       &   -13.6***  &         &  -13.5  & & -15.1*\\
                &       &   (8.1)    &          &   (8.5)  &&(8.8)\\
$Const$       & 51.9***   &   86.7***& 52.8*** &  87.3***   & 51.1***&89.7***\\
             &  (4.9)    &  (21.5)    & (5.2)  &    (22.3)   & (6.1)&(23.5)\\ 
        
        \midrule
N      (individuals)&459 &  459 & 441&  441 & 101 & 101\\
$R^2$          &0.01  &    0.02      & 0.01  &0.02       & 0.02 &0.05\\

\bottomrule
\end{tabular}
\\
\textbf{Dep. Variable}: $time_{t,u,i}$ (bus trips)\\

\begin{tabular}{c | c c c c c c }
\toprule
\textbf{Ind. Variable} & $trips$ &  & $respondents$ & & $cells$ & \\ 
\midrule
$CA_i(bus)$  & -0.09***&   -0.05***   &   -0.09***  & -0.05***   & -0.09*** &-0.06\\
               & (0.01)  &   (0.01)   &    (0.01) & (0.01)      & (0.01)&(0.02)\\
$stratum_i$     &       &   -0.06***  &         &  -0.06***  & & -0.05***\\
                &       &   (0.01)    &          &   (0.01)  &&(0.01)\\
$Const$       & 1.90***   &   2.06***& 1.90*** &  2.06***   & 1.93***&2.05***\\
             &  (0.01)    &  (0.03)    & (0.01)  &    (0.03)   & (0.01)&(0.04)\\ 
        
        \midrule
N      (individuals)&1356 &  1356 &  1349&  1349 & 117 & 117\\
$R^2$          &0.07  &    0.09      & 0.07  &0.09       & 0.27 &0.33\\

\bottomrule
\end{tabular}
\\
\textbf{Dep. Variable}: $log \;time_{t,u,i}$ (automobile trips)\\

\begin{tabular}{c | c c c c c c }
\toprule
\textbf{Ind. Variable} & $trips$ &  & $respondents$ & & $cells$ & \\ 
\midrule
$CA_i(auto)$  & -0.05***&   -0.04***   &   -0.06***  & -0.04***   & -0.06*** &-0.02\\
               & (0.01)  &   (0.01)   &    (0.01) & (0.01)      & (0.02)&(0.02)\\
$stratum_i$     &       &   -0.01*  &         &  -0.02**  & & -0.05***\\
                &       &   (0.01)    &          &   (0.01)  &&(0.02)\\
$Const$      & 1.55***   &   1.59***& 1.56*** &  1.61***   & 1.59***&1.72***\\
             &  (0.01)    &  (0.02)    & (0.01)  &    (0.03)   & (0.02)&(0.05)\\ 
        
        \midrule
N      (individuals)&2410 &  2410 &  2278&  2278 & 117 & 117\\
$R^2$          &0.01  &    0.01      & 0.01  &0.01       & 0.08 &0.14\\

\bottomrule
\end{tabular}
\label{table:trips}
\end{table}
%\end{boxedverbatim}
\end{center}
%\caption{Example table layout.\label{F2}}
%\end{figure}

==> tables/mode_new.tex <==

%\begin{figure}
%\setlength{\fboxsep}{0pt}%
%\setlength{\fboxrule}{0pt}%
%\begin{boxedverbatim}
\begin{table}

\scriptsize\sf\centering
\caption{Effects on $Pr(walk)$, $Pr(bike)$ (Logistic regression)}

\begin{tabular}{c | c c }
\toprule
& $walk$ & $walk$ \\
\toprule
\textbf{Ind. Variable} & (1a) & (1b)  \\ 
\midrule
$access(poly)$  & -4.58***	&-3.10*** \\
               &(0.351)&(0.39)	 \\
$access(walk)$  &  0.92*** & 1.17***    \\
&    (0.12)    &(0.12) \\
$access(bike)$  &   &    \\
&   &     \\
$homes(grav)$  &   5.82E-7***&2.08E-7\\
&      (0.53e-7)&(0.68E-7)\\
$stratum$  & &-0.30***	\\
&       &(0.03)	\\
$stratum\times access$  &   &0.02\\
&   &(0.02)\\
$const$&-1.81***&-1.15***\\
&(0.17)&(0.19)\\
Weekday FE & -0.11***	&-0.10***\\
Searching FE & 2.02***&(0.04)\\
Eating FE&  2.62***&2.02***\\
Shopping FE& 3.14***&2.67***\\
Errand FE&  1.36***&3.15***\\
Recreational FE&  2.12***&1.37***\\
Religious FE&  2.21***&2.14***\\
Physical FE& 3.22***&2.22***\\
Age&  0.01***&3.27***\\
Female FE&  0.42***&0.43***\\
\midrule
N  (individuals)&15133&	15133\\
Pseudo-$R^2$&0.20&0.20 \\

\bottomrule
\end{tabular}

\label{table:walk}
\end{table}
%\end{boxedverbatim}
%\end{center}
%\caption{Example table layout.\label{F2}}


==> tables/new_table.tex <==

%\begin{figure}
%\setlength{\fboxsep}{0pt}%
%\setlength{\fboxrule}{0pt}%
\begin{center}
%\begin{boxedverbatim}
\begin{table}

\scriptsize\sf\centering
\caption{Effects of $access$ on trip behavior}
\textbf{Dep. Variable}: $time_{t}$ (bus trips)\\

\begin{tabular}{c | c c c c c c c c }
\toprule
&&&&Respondent subset &&&&\\
 & (all respondents) & (all respondents)  & (low SES gp) &(low SES gp) & (middle SES gp) & (middle SES gp) & (high SES gp)&(high SES gp)\\ 
\midrule
&&&& $Optimal$ $\lambda$ &&&&\\
& & & & & & & &\\
\midrule

\textbf{Ind. Variable} & Model I &Model II & Model I &Model I&Model II & &Model I  &Model II\\

$access(\lambda)$  & 1  & 2    &1l   &2l&1m&2m&1h&2h  \\
              & 1  & 2    &1l   &2l&1m&2m&1h&2h \\
$stratum_z$     & 1  & 2    &1l   &2l&1m&2m&1h&2h \\
                & 1  & 2    &1l   &2l&1m&2m&1h&2h \\
$homes+jobs$     & 1  & 2    &1l   &2l&1m&2m&1h&2h \\
                & 1  & 2    &1l   &2l&1m&2m&1h&2h \\
Weekday FE & 1  & 2    &1l   &2l&1m&2m&1h&2h \\

$Const$           & 1  & 2    &1l   &2l&1m&2m&1h&2h \\
                & 1  & 2    &1l   &2l&1m&2m&1h&2h \\
        \midrule
T (trips) & 1  & 2    &1l   &2l&1m&2m&1h&2h \\
             
$R^2$         $stratum_z$     & 1  & 2    &1l   &2l&1m&2m&1h&2h \\

\bottomrule
\end{tabular}
\\

\textbf{Dep. Variable}: $time_{t,u,i}$ (walking)\\

\begin{tabular}{c | c c c c c c }
\toprule
\textbf{Ind. Variable} & $trips$ &  & $respondents$ & & $cells$ & \\ 
\midrule
$CA_i(walk)$  & 1.0&     1.0   &   0.9  &  0.8   & -0.5 &-0.9\\
               & (0.7)  &   (1.0)   &    (0.7) & (1.0)      & (0.8)&(1.0)\\
$stratum_i$     &       &   -0.0  &         &  0.0  & & 0.6\\
                &       &   (0.7)    &          &   (0.8)  &&(0.8)\\
$Const$       & 23.8***   &   23.8***    & 24.0*** &   23.8***   & 23.4***&22.0\\
             &  (0.5)    &  (1.9)    & (0.5)  &    (2.0)   & (0.6)&(2.0)\\ 
        
        \midrule
N      (individuals)&6193 &  6193 &  12286&  12286 & 119 & 119\\
$R^2$          &0.00  &    0.00      & 0.00  &0.00       & 0.00 &0.01\\

\bottomrule
\end{tabular}
\\
\textbf{Dep. Variable}: $time_{t,u,i}$ (bike trips)\\

\begin{tabular}{c | c c c c c c }
\toprule
\textbf{Ind. Variable} & $trips$ &  & $respondents$ & & $cells$ & \\ 
\midrule
$CA_i(bike)$  & 13.4**&   20.1***   &   13.5**  & 20.5***   & 11.4 &20.1**\\
               & (6.0)  &   (7.2)   &    (6.3) & (7.7)      & (7.5)&(9.0)\\
$stratum_i$     &       &   -13.6***  &         &  -13.5  & & -15.1*\\
                &       &   (8.1)    &          &   (8.5)  &&(8.8)\\
$Const$       & 51.9***   &   86.7***& 52.8*** &  87.3***   & 51.1***&89.7***\\
             &  (4.9)    &  (21.5)    & (5.2)  &    (22.3)   & (6.1)&(23.5)\\ 
        
        \midrule
N      (individuals)&459 &  459 & 441&  441 & 101 & 101\\
$R^2$          &0.01  &    0.02      & 0.01  &0.02       & 0.02 &0.05\\

\bottomrule
\end{tabular}
\\
\textbf{Dep. Variable}: $time_{t,u,i}$ (bus trips)\\

\begin{tabular}{c | c c c c c c }
\toprule
\textbf{Ind. Variable} & $trips$ &  & $respondents$ & & $cells$ & \\ 
\midrule
$CA_i(bus)$  & -0.09***&   -0.05***   &   -0.09***  & -0.05***   & -0.09*** &-0.06\\
               & (0.01)  &   (0.01)   &    (0.01) & (0.01)      & (0.01)&(0.02)\\
$stratum_i$     &       &   -0.06***  &         &  -0.06***  & & -0.05***\\
                &       &   (0.01)    &          &   (0.01)  &&(0.01)\\
$Const$       & 1.90***   &   2.06***& 1.90*** &  2.06***   & 1.93***&2.05***\\
             &  (0.01)    &  (0.03)    & (0.01)  &    (0.03)   & (0.01)&(0.04)\\ 
        
        \midrule
N      (individuals)&1356 &  1356 &  1349&  1349 & 117 & 117\\
$R^2$          &0.07  &    0.09      & 0.07  &0.09       & 0.27 &0.33\\

\bottomrule
\end{tabular}
\\
\textbf{Dep. Variable}: $log \;time_{t,u,i}$ (automobile trips)\\

\begin{tabular}{c | c c c c c c }
\toprule
\textbf{Ind. Variable} & $trips$ &  & $respondents$ & & $cells$ & \\ 
\midrule
$CA_i(auto)$  & -0.05***&   -0.04***   &   -0.06***  & -0.04***   & -0.06*** &-0.02\\
               & (0.01)  &   (0.01)   &    (0.01) & (0.01)      & (0.02)&(0.02)\\
$stratum_i$     &       &   -0.01*  &         &  -0.02**  & & -0.05***\\
                &       &   (0.01)    &          &   (0.01)  &&(0.02)\\
$Const$      & 1.55***   &   1.59***& 1.56*** &  1.61***   & 1.59***&1.72***\\
             &  (0.01)    &  (0.02)    & (0.01)  &    (0.03)   & (0.02)&(0.05)\\ 
        
        \midrule
N      (individuals)&2410 &  2410 &  2278&  2278 & 117 & 117\\
$R^2$          &0.01  &    0.01      & 0.01  &0.01       & 0.08 &0.14\\

\bottomrule
\end{tabular}
\label{table:trips}
\end{table}
%\end{boxedverbatim}
\end{center}
%\caption{Example table layout.\label{F2}}
%\end{figure}

==> tables/new_walk.tex <==
\begin{center}
%\begin{boxedverbatim}
\begin{table}

\tiny\sf\centering
\caption{Effects of $access$ on propensity towalk}
\textbf{Dep. Variable}: $Pr(walk)_t$\\

\begin{tabular}{c | c c| c c| c c| c c }
\toprule

Respondents & {\bf(all)} &  & {\bf(low SES)} & & {\bf(middle SES)} && {\bf(high SES)}&\\ 

\midrule
\textbf{Ind. Variable} & Model I &Model II & Model I&Model II &Model I&Model II & Model I  &Model II\\
 \midrule \\[-1.8ex]


$access_{z(t)}$ & 3.94$^{***}$ & 4.54$^{***}$ & 1.64$^{}$ & 6.29$^{***}$ & 4.29$^{***}$ & 3.05$^{***}$ & 26.75$^{***}$ & 16.18$^{***}$ \\  & (0.97) & (0.84) & (1.43) & (1.67) & (1.44) & (1.08) & (5.40) & (3.12) \\ $homes+jobs_{z(t)}$ & & -0.00$^{**}$ & & -0.00$^{***}$ & & 0.00$^{}$ & & 0.00$^{*}$ \\  & & (0.00) & & (0.00) & & (0.00) & & (0.00) \\
$stratum_{z(t)}$ & -0.18$^{***}$ & -0.18$^{***}$ & & & & & & \\  & (0.04) & (0.04) & & & & & & \\


Intercept & -2.57$^{***}$ & -2.29$^{***}$ & -2.86$^{***}$ & -2.20$^{***}$ & -3.22$^{***}$ & -3.54$^{***}$ & -6.90$^{***}$ & -7.18$^{***}$ \\  & (0.20) & (0.23) & (0.29) & (0.34) & (0.36) & (0.43) & (1.21) & (1.67) \\
own car$_t$ & -0.67$^{***}$ & -0.65$^{***}$ & -0.74$^{***}$ & -0.72$^{***}$ & -0.69$^{***}$ & -0.69$^{***}$ & 0.02$^{}$ & -0.01$^{}$ \\  & (0.08) & (0.08) & (0.14) & (0.14) & (0.12) & (0.12) & (0.41) & (0.41) \\
weekend$_t$ & -0.15$^{*}$ & -0.14$^{*}$ & -0.01$^{}$ & 0.01$^{}$ & -0.17$^{}$ & -0.17$^{}$ & -0.83$^{***}$ & -0.94$^{***}$ \\  & (0.08) & (0.08) & (0.13) & (0.13) & (0.12) & (0.12) & (0.30) & (0.30) \\
female$_t$ & 0.49$^{***}$ & 0.49$^{***}$ & 0.50$^{***}$ & 0.49$^{***}$ & 0.50$^{***}$ & 0.50$^{***}$ & 0.48$^{*}$ & 0.55$^{*}$ \\  & (0.08) & (0.08) & (0.13) & (0.13) & (0.12) & (0.12) & (0.29) & (0.29) \\ 
age$_t$& 0.01$^{***}$ & 0.01$^{***}$ & 0.01$^{***}$ & 0.01$^{***}$ & 0.01$^{***}$ & 0.01$^{***}$ & 0.03$^{***}$ & 0.02$^{***}$ \\  & (0.00) & (0.00) & (0.00) & (0.00) & (0.00) & (0.00) & (0.01) & (0.01) \\
 shop$_t$ & 3.01$^{***}$ & 3.03$^{***}$ & 3.38$^{***}$ & 3.42$^{***}$ & 2.95$^{***}$ & 2.96$^{***}$ & 1.46$^{***}$ & 1.46$^{***}$ \\  & (0.14) & (0.14) & (0.22) & (0.22) & (0.21) & (0.21) & (0.45) & (0.45) \\ errand$_t$ & 1.32$^{***}$ & 1.31$^{***}$ & 1.35$^{***}$ & 1.36$^{***}$ & 1.37$^{***}$ & 1.38$^{***}$ & 0.88$^{*}$ & 0.94$^{**}$ \\  & (0.14) & (0.14) & (0.21) & (0.21) & (0.22) & (0.22) & (0.47) & (0.48) \\ recreation$_t$ & 2.74$^{***}$ & 2.76$^{***}$ & 2.70$^{***}$ & 2.76$^{***}$ & 2.81$^{***}$ & 2.82$^{***}$ & 2.70$^{***}$ & 2.59$^{***}$ \\  & (0.20) & (0.20) & (0.32) & (0.32) & (0.27) & (0.27) & (0.71) & (0.72) \\ religion$_t$ & 1.93$^{***}$ & 1.93$^{***}$ & 1.64$^{***}$ & 1.67$^{***}$ & 2.25$^{***}$ & 2.27$^{***}$ & 1.51$^{*}$ & 1.58$^{*}$ \\  & (0.22) & (0.22) & (0.33) & (0.33) & (0.32) & (0.32) & (0.88) & (0.90) \\ physical$_t$ & 3.11$^{***}$ & 3.12$^{***}$ & 3.45$^{***}$ & 3.47$^{***}$ & 3.09$^{***}$ & 3.10$^{***}$ & 2.18$^{***}$ & 2.17$^{***}$ \\  & (0.19) & (0.19) & (0.34) & (0.35) & (0.27) & (0.27) & (0.54) & (0.54) \\ search$_t$ & 2.14$^{***}$ & 2.13$^{***}$ & 2.44$^{***}$ & 2.48$^{***}$ & 1.95$^{***}$ & 1.96$^{***}$ & 0.61$^{}$ & 0.80$^{}$ \\  & (0.21) & (0.21) & (0.29) & (0.29) & (0.36) & (0.36) & (1.08) & (1.07) \\ dine$_t$ & 2.88$^{***}$ & 2.84$^{***}$ & 3.06$^{***}$ & 3.02$^{***}$ & 2.93$^{***}$ & 2.94$^{***}$ & 1.65$^{***}$ & 1.56$^{***}$ \\  & (0.22) & (0.22) & (0.38) & (0.39) & (0.32) & (0.32) & (0.53) & (0.54) \\    \bottomrule \\[-1.8ex] Obs. & 3,425 & 3,425 & 1,504 & 1,504 & 1,626 & 1,626 & 295 & 295 \\ Pseudo-$R^2$ &.20  & .20 &.23  &.24  & .19 &.19  &.18  &  .20
 \\ \bottomrule  


\end{tabular}
\label{pr_walk}
\end{table}
\end{center}

==> tables/new_walk_heckman.tex <==
\begin{center}
%\begin{boxedverbatim}
\begin{table}

\tiny\sf\centering
\caption{Effects of $access$ on propensity to walk}
\textbf{Dep. Variable}: $Pr(walk)_t$\\

\begin{tabular}{c | c c| c c| c c| c c }
\toprule

Respondents & {\bf(all)} &  & {\bf(low SES)} & & {\bf(middle SES)} && {\bf(high SES)}&\\ 

\midrule
\textbf{Ind. Variable} & Model I &Model II & Model I&Model II &Model I&Model II & Model I  &Model II\\
 \midrule \\[-1.8ex]

        $\log\;access(0.5\;km)_{z(t)}$ &   0.06$^{***}$ &   0.27$^{***}$ &   0.12$^{***}$ &   0.28$^{***}$ &    0.1$^{***}$ &   0.16$^{***}$ &   0.54$^{***}$ &   0.44$^{***}$ \\
                     &         (0.01) &         (0.02) &         (0.02) &         (0.03) &         (0.04) &         (0.04) &         (0.08) &         (0.11) \\
    $stratum_{z(t)}$ &          &  -0.13$^{***}$ &           &          &        &         &          &     \\
                     &        &         (0.01) &          &          &          &       &           &        \\
 $homes+jobs_{z(t)}$ &            &  -0.16$^{***}$ &           &  -0.23$^{***}$ &         &  -0.11$^{***}$ &          &           0.21 \\
                     &        &         (0.02) &        &         (0.03) &          &         (0.03) &          &         (0.13) \\
           Intercept &  -1.17$^{***}$ &   3.79$^{***}$ &  -1.05$^{***}$ &    5.3$^{***}$ &  -1.27$^{***}$ &      1.7$^{*}$ &           0.13 &          -5.76 \\
                     &         (0.06) &         (0.63) &          (0.1) &         (0.89) &          (0.1) &         (0.97) &         (0.26) &          (3.6) \\
         own car$_t$ &  -0.45$^{***}$ &  -0.36$^{***}$ &  -0.27$^{***}$ &  -0.27$^{***}$ &  -0.46$^{***}$ &  -0.45$^{***}$ &  -0.37$^{***}$ &  -0.36$^{***}$ \\
                     &         (0.02) &         (0.02) &         (0.04) &         (0.04) &         (0.03) &         (0.03) &         (0.11) &         (0.11) \\
         weekend$_t$ &  -0.06$^{***}$ &   -0.05$^{**}$ &          -0.05 &          -0.05 &   -0.07$^{**}$ &   -0.07$^{**}$ &          -0.03 &          -0.02 \\
                     &         (0.02) &         (0.02) &         (0.04) &         (0.04) &         (0.03) &         (0.03) &         (0.09) &         (0.09) \\
          female$_t$ &   0.24$^{***}$ &   0.23$^{***}$ &   0.27$^{***}$ &   0.26$^{***}$ &   0.23$^{***}$ &   0.23$^{***}$ &     0.14$^{*}$ &            0.1 \\
                     &         (0.02) &         (0.02) &         (0.04) &         (0.04) &         (0.03) &         (0.03) &         (0.08) &         (0.08) \\
             age$_t$ &    0.0$^{***}$ &   0.01$^{***}$ &    0.0$^{***}$ &    0.0$^{***}$ &   0.01$^{***}$ &   0.01$^{***}$ &            0.0 &      0.0$^{*}$ \\
                     &          (0.0) &          (0.0) &          (0.0) &          (0.0) &          (0.0) &          (0.0) &          (0.0) &          (0.0) \\
            dine$_t$ &   1.53$^{***}$ &   1.59$^{***}$ &   1.84$^{***}$ &   1.85$^{***}$ &   1.63$^{***}$ &   1.63$^{***}$ &   0.73$^{***}$ &   0.75$^{***}$ \\
                     &         (0.06) &         (0.06) &         (0.12) &         (0.13) &         (0.08) &         (0.08) &         (0.17) &         (0.17) \\
          errand$_t$ &   0.78$^{***}$ &   0.79$^{***}$ &   0.71$^{***}$ &   0.73$^{***}$ &   0.86$^{***}$ &   0.87$^{***}$ &   0.69$^{***}$ &   0.68$^{***}$ \\
                     &         (0.04) &         (0.04) &         (0.06) &         (0.06) &         (0.05) &         (0.05) &         (0.14) &         (0.14) \\
      recreation$_t$ &    1.2$^{***}$ &   1.27$^{***}$ &   1.49$^{***}$ &   1.51$^{***}$ &   1.19$^{***}$ &    1.2$^{***}$ &   0.73$^{***}$ &   0.74$^{***}$ \\
                     &         (0.05) &         (0.05) &         (0.09) &         (0.09) &         (0.07) &         (0.07) &         (0.17) &         (0.17) \\
        shopping$_t$ &   1.88$^{***}$ &    1.9$^{***}$ &   2.07$^{***}$ &   2.09$^{***}$ &   1.87$^{***}$ &   1.87$^{***}$ &   1.05$^{***}$ &   1.04$^{***}$ \\
                     &         (0.04) &         (0.04) &         (0.06) &         (0.06) &         (0.05) &         (0.05) &         (0.13) &         (0.13) \\
       religious$_t$ &   1.29$^{***}$ &    1.3$^{***}$ &   1.28$^{***}$ &   1.32$^{***}$ &   1.36$^{***}$ &   1.35$^{***}$ &   0.85$^{***}$ &   0.86$^{***}$ \\
                     &         (0.06) &         (0.06) &         (0.11) &         (0.11) &         (0.09) &         (0.09) &         (0.25) &         (0.25) \\
        physical$_t$ &    1.9$^{***}$ &   1.95$^{***}$ &   1.84$^{***}$ &   1.85$^{***}$ &   2.04$^{***}$ &   2.05$^{***}$ &   1.49$^{***}$ &   1.51$^{***}$ \\
                     &         (0.05) &         (0.05) &         (0.08) &         (0.08) &         (0.07) &         (0.07) &         (0.16) &         (0.16) \\
         search$_t$ &   1.21$^{***}$ &   1.19$^{***}$ &   1.27$^{***}$ &   1.26$^{***}$ &   1.25$^{***}$ &   1.25$^{***}$ &           0.05 &           0.08 \\
                     &         (0.06) &         (0.06) &         (0.08) &         (0.08) &         (0.09) &         (0.09) &          (0.3) &          (0.3) \\\bottomrule \\[-1.8ex] 
                 Obs &        15133 &        15133 &         6005&         6005 &         7932 &         7932 &         1196 &         1196 \\
        Pseudo-$R^2$ &           0.21 &           0.21 &           0.24 &           0.25 &           0.21 &           0.21 &           0.13 &           0.13 
\\ \bottomrule  


\end{tabular}
\label{pr_walk}
\end{table}
\end{center}

==> tables/ols_time.tex <==

%\begin{figure}
%\setlength{\fboxsep}{0pt}%
%\setlength{\fboxrule}{0pt}%

%\begin{boxedverbatim}
\begin{table}

\scriptsize\sf\centering
\caption{Effects of accessibility on trip time}
A. \textbf{Dep. Variable}: polymodal $log \;time_{t}$ (OLS)\\

\begin{tabular}{c | c c c c c c }
\toprule
\textbf{Ind. Variable} & $trips$ &  &  & \\ 
\midrule
$CA_i(poly)$  & -0.02***  &     -0.00   &   -0.03***  &  -0.01**  \\
               & (0.01)  &   (0.01)   &    (0.00) & (0.01)     \\
$stratum_i$     &       &   -0.02***  &           &  -0.03**  \\
                &       &   (0.01)    &          &   (0.01)  \\
$Const$       & 1.41***   &   1.46***  &  1.65*** &   1.73***   \\
             &  (0.01)    &  (0.02)    & (0.03)  &    (0.03)   \\ 
Mode FE           &            &           &  x       &x\\     
        \midrule
N      (individuals)&9829 &  9829 & 9829 &  9829\\
$R^2$          &0.00  &    0.00      & 0.37  &0.37 \\

\bottomrule
\end{tabular}
\\

B. \textbf{Dep. Variable}: walking $log\;time_{t,u,i}$ (OLS for $trips$, $respondents$; WLS for $cells$)\\

\begin{tabular}{c | c c c c c c }
\toprule
\textbf{Ind. Variable} & $trips$  & & $respondents$ &  & $cells$ &  \\ 
\midrule
$CA_i(walk)$  & 0.00&     -0.00   &   0.00  &  -0.00   & 0.0 &0.00\\
               & (0.01)  &   (0.01)   &    (0.01) & (0.01)      & (0.01)&(0.01)\\
$stratum_i$     &       &   0.00  &         &  0.00  & & 0.00\\
                &       &   (0.01)    &          &   (0.01)  &&(0.01)\\
$Const$       & 1.13***   &   1.13***    & 1.14*** &   1.13***   & 1.14***&1.13***\\
             &  (0.01)    &  (0.02)    & (0.01)  &    (0.02)   & (0.01)&(0.03)\\ 
        
        \midrule
N      (individuals)&4667 &  4667&  4248&  4248 & 117& 117\\
$R^2$          &0.00  &    0.00      & 0.00  &0.00       & 0.00 &0.00\\

\bottomrule
\end{tabular}
\\
C. \textbf{Dep. Variable}: bike $log\;time_{t,u,i}$ (OLS for $trips$, $respondents$; WLS for $cells$)\\

\begin{tabular}{c | c c c c c c }
\toprule
\textbf{Ind. Variable} & $trips$ &  & $respondents$ & & $cells$ & \\ 
\midrule
$CA_i(bike)$  & 0.06**&   0.10***   &   0.07**  & 0.11***   & 0.07** &0.11***\\
               & (0.03)  &   (0.04)   &    (0.03) & (0.04)      & (0.03)&(0.04)\\
$stratum_i$     &       &   -0.06*  &         &  -0.07*  & & -0.07\\
                &       &   (0.04)    &          &   (0.04)  &&(0.04)\\
$Const$       & 1.31***   &   1.47***& 1.31*** &  1.49***   & 1.31***&1.49***\\
             &  (0.02)    &  (0.10)    & (0.02)  &    (0.10)   & (0.03)&(0.11)\\ 
        
        \midrule
N      (individuals)&356 &  356 & 350&  350 & 93 & 93\\
$R^2$          &0.01  &    0.02      & 0.01  &0.02       & 0.04 &0.12\\

\bottomrule
\end{tabular}
\\
D. \textbf{Dep. Variable}: bus $log\;time_{t,u,i}$ (OLS for $trips$, $respondents$; WLS for $cells$)\\

\begin{tabular}{c | c c c c c c }
\toprule
\textbf{Ind. Variable} & $trips$ &  & $respondents$ & & $cells$ & \\ 
\midrule
$CA_i(bus)$  & -0.07***&   -0.03***   &   -0.07***  & -0.03***   & -0.07*** &-0.03**\\
               & (0.01)  &   (0.01)   &    (0.01) & (0.01)      & (0.01)&(0.01)\\
$stratum_i$     &       &   -0.08***  &         &  -0.08***  & & -0.08***\\
                &       &   (0.01)    &          &   (0.01)  &&(0.01)\\
$Const$       & 1.75***   &   1.96***& 1.75*** &  1.96***   & 1.75***&1.96***\\
             &  (0.01)    &  (0.02)    & (0.01)  &    (0.02)   & (0.01)&(0.04)\\ 
        
        \midrule
N      (individuals)&3092 &  3092& 3012&  3012& 117 & 117\\
$R^2$          &0.05  &    0.07      & 0.05  &0.07       & 0.32 &0.47\\

\bottomrule
\end{tabular}
\\
\textbf{Dep. Variable}: automobile $log \;time_{t,u,i}$ (OLS for $trips$, $respondents$; WLS for $cells$)\\

\begin{tabular}{c | c c c c c c }
\toprule
E. \textbf{Ind. Variable} & $trips$ &  & $respondents$ & & $cells$ & \\ 
\midrule
$CA_i(auto)$  & -0.06***&   -0.04**   &   -0.06***  & -0.04**   & -0.07*** &-0.04*\\
               & (0.01)  &   (0.02)   &    (0.01) & (0.02)      & (0.02)&(0.02)\\
$stratum_i$     &       &   -0.03***  &         &  -0.03***  & & -0.03**\\
                &       &   (0.01)    &          &   (0.01)  &&(0.01)\\
$Const$      & 1.54***   &   1.63***& 1.55*** &  1.64***   & 1.55***&1.64***\\
             &  (0.01)    &  (0.03)    & (0.01)  &    (0.04)   & (0.01)&(0.04)\\ 
        
        \midrule
N      (individuals)&1509 &  1509 &  1432&  1432 & 115 & 115\\
$R^2$          &0.01  &    0.02      & 0.01  &0.01       & 0.10 &0.13\\

\bottomrule
\end{tabular}
\label{table:trips}
\end{table}
%\end{boxedverbatim}
%\end{center}
%\caption{Example table layout.\label{F2}}


==> tables/stargazer_bus.tex <==
\begin{center}
\begin{table}
\tiny
\caption{Effects of amenity accessibility on bus trip duration}
\textbf{Dep. Variable}: $\log\;duration_{t}$ (bus trips)\\

\begin{tabular}{c | c c| c c |c c| c c }
Respondent subset & (all) & (all) &(low SES)&(low SES)&(middle SES)&(middle SES)&(high SES)&(high SES)\\

\toprule
Model & (I) & (II) & (I) & (II) & (I) & (II) & (I) & (II) \\
\toprule 
 $\log\;access(1.5\;km)_{z(t)}$ & -0.19$^{***}$ & -0.26$^{***}$ & -0.20$^{***}$ & -0.25$^{***}$ & -0.27$^{***}$ & -0.41$^{***}$ & -1.11$^{**}$ & -1.32$^{**}$ \\  & (0.03) & (0.05) & (0.04) & (0.07) & (0.08) & (0.10) & (0.40) & (0.43) \\ $homes+jobs_{z(t)}$ & & 0.00$^{*}$ & & 0.00$^{}$ & & 0.00$^{**}$ & & 0.00$^{}$ \\  & & (0.00) & & (0.00) & & (0.00) & & (0.00)
 \\ $stratum_{z(t)}$ & -0.05$^{**}$ & -0.04$^{**}$ & & & & & & \\  & (0.02) & (0.02) & & & & & & \\ 
Intercept & 3.52$^{***}$ & 3.09$^{***}$ & 3.36$^{***}$ & 3.06$^{***}$ & 3.32$^{***}$ & 2.61$^{***}$ & 2.54$^{***}$ & 1.05$^{}$ \\  
& (0.17) & (0.29) & (0.18) & (0.37) & (0.29) & (0.44) & (0.82) & (1.50) \\
weekend$_t$ & 0.02$^{}$ & 0.02$^{}$ & 0.07$^{}$ & 0.07$^{}$ & -0.03$^{}$ & -0.04$^{}$ & -0.31$^{**}$ & -0.31$^{**}$ \\
female$_t$ & -0.04$^{}$ & -0.04$^{}$ & -0.02$^{}$ & -0.02$^{}$ & -0.09$^{*}$ & -0.10$^{*}$ & 0.12$^{}$ & 0.11$^{}$ \\ age$_t$& 0.00$^{}$ & 0.00$^{}$ & 0.00$^{}$ & 0.00$^{}$ & -0.00$^{}$ & -0.00$^{}$ & -0.01$^{}$ & -0.00$^{}$  \\ 
Intermunicipal$_t$ & -0.05$^{}$ & -0.02$^{}$ & -0.25$^{}$ & -0.22$^{}$ & 0.11$^{}$ & 0.15$^{}$ & & \\  
SITP Provisional$_t$ & 0.21$^{**}$ & 0.23$^{**}$ & 0.20$^{*}$ & 0.21$^{*}$ & 0.22$^{}$ & 0.23$^{}$ & & 
\\ SITP Zonal$_t$ & 0.37$^{***}$ & 0.38$^{***}$ & 0.34$^{***}$ & 0.36$^{***}$ & 0.36$^{*}$ & 0.35$^{*}$ & 0.09$^{}$ & 0.14$^{}$ \\
TransMilenio$_t$ & 0.52$^{***}$ & 0.55$^{***}$ & 0.53$^{***}$ & 0.55$^{***}$ & 0.45$^{**}$ & 0.49$^{**}$ & -0.12$^{}$ & -0.07$^{}$ \\ 
shop$_t$ & -0.23$^{***}$ & -0.24$^{***}$ & -0.45$^{***}$ & -0.45$^{***}$ & -0.09$^{}$ & -0.09$^{}$ & 0.19$^{}$ & 0.28$^{*}$ 
\\ errand$_t$ & -0.09$^{**}$ & -0.09$^{**}$ & -0.15$^{***}$ & -0.15$^{***}$ & -0.03$^{}$ & -0.03$^{}$ & 0.01$^{}$ & 0.06$^{}$ 
\\ recreation$_t$ & -0.14$^{}$ & -0.13$^{}$ & -0.32$^{**}$ & -0.32$^{**}$ & -0.02$^{}$ & 0.00$^{}$ & 0.59$^{*}$ & 0.57$^{*}$ 
\\ religion$_t$ & -0.10$^{}$ & -0.11$^{}$ & -0.43$^{***}$ & -0.43$^{***}$ & 0.21$^{}$ & 0.19$^{}$ & 0.78$^{**}$ & 0.79$^{**}$ \\ 
physical$_t$ & -0.34$^{**}$ & -0.34$^{**}$ & -0.45$^{**}$ & -0.45$^{**}$ & -0.20$^{}$ & -0.19$^{}$ & -0.00$^{}$ & -0.00$^{}$ 
\\ search$_t$ & -0.29$^{**}$ & -0.29$^{***}$ & -0.30$^{**}$ & -0.30$^{**}$ & -0.20$^{}$ & -0.20$^{}$ & -0.00$^{}$ & -0.00$^{}$ 
\\ dine$_t$ & -0.02$^{}$ & -0.02$^{}$ & 0.10$^{}$ & 0.09$^{}$ & 0.12$^{}$ & 0.14$^{}$ & -0.95$^{***}$ & -0.98$^{***}$ 


\\ \bottomrule \\[-1.8ex] Obs. & 856 & 856 & 461 & 461 & 371 & 371 & 24 & 24 \\ $R^2$ & 0.16 & 0.17 & 0.23 & 0.23 & 0.11 & 0.12 & 0.80 & 0.82 \\ Adjusted $R^2$ & 0.15 & 0.15 & 0.20 & 0.20 & 0.07 & 0.08 & 0.62 & 0.63 \\ 
 \end{tabular}
\label{trips_bus}
\end{table}
\end{center}

==> tables/stargazer_car.tex <==

\begin{center}
\begin{table}
\tiny
\caption{Effects of amenity accessibility on car/motorcycle trip duration}
\textbf{Dep. Variable}: $\log\;duration_{t}$ (car/moto trips)\\

\begin{tabular}{c | c c| c c| c c |c c }
Respondent subset & (all) & (all) &(low SES)&(low SES)&(middle SES)&(middle SES)&(high SES)&(high SES)\\

\toprule
Model & (I) & (II) & (I) & (II) & (I) & (II) & (I) & (II) \\
\toprule 


$\log\;access(1.5\;km)_{z(t)}$ & -0.23$^{***}$ & -0.31$^{**}$ & -0.03$^{}$ & -0.28$^{}$ & -0.50$^{***}$ & -0.62$^{***}$ & 0.55$^{}$ & 0.86$^{*}$ \\  & (0.08) & (0.13) & (0.12) & (0.19) & (0.14) & (0.20) & (0.44) & (0.47) \\ $homes+jobs_{z(t)}$ & & 0.00$^{}$ & & 0.00$^{*}$ & & 0.00$^{}$ & & -0.00$^{*}$ \\  & & (0.00) & & (0.00) & & (0.00) & & (0.00) \\
$stratum_{z(t)}$ & -0.06$^{**}$ & -0.05$^{}$ & & & & & & \\  & (0.03) & (0.03) & & & & & & \\
Intercept & 3.35$^{***}$ & 2.92$^{***}$ & 3.58$^{***}$ & 2.34$^{***}$ & 2.79$^{***}$ & 2.26$^{***}$ & 4.21$^{***}$ & 5.92$^{***}$ \\  & (0.27) & (0.55) & (0.45) & (0.87) & (0.35) & (0.72) & (0.89) & (1.28) \\ 
weekend$_t$ & 0.07$^{}$ & 0.07$^{}$ & -0.02$^{}$ & -0.03$^{}$ & 0.11$^{}$ & 0.11$^{}$ & 0.07$^{}$ & 0.04$^{}$  \\
female$_t$ & -0.00$^{}$ & -0.00$^{}$ & -0.03$^{}$ & -0.01$^{}$ & -0.01$^{}$ & -0.01$^{}$ & -0.03$^{}$ & -0.01$^{}$ \\ 
age$_t$& 0.00$^{}$ & 0.00$^{}$ & 0.00$^{}$ & 0.00$^{}$ & -0.00$^{}$ & -0.00$^{}$ & 0.01$^{*}$ & 0.01$^{*}$ \\
motorcycle$_t$ & -0.29$^{***}$ & -0.29$^{***}$ & -0.24$^{}$ & -0.21$^{}$ & -0.27$^{}$ & -0.29$^{}$ & -0.58$^{*}$ & -0.47$^{}$ \\   shop$_t$ & -0.50$^{***}$ & -0.49$^{***}$ & -0.12$^{}$ & -0.13$^{}$ & -0.76$^{***}$ & -0.75$^{***}$ & -0.38$^{**}$ & -0.37$^{**}$  \\ errand$_t$ & -0.17$^{*}$ & -0.17$^{*}$ & -0.07$^{}$ & -0.10$^{}$ & -0.34$^{***}$ & -0.33$^{***}$ & -0.06$^{}$ & -0.02$^{}$  \\ recreation$_t$ & -0.35$^{**}$ & -0.36$^{**}$ & -0.42$^{}$ & -0.52$^{*}$ & -0.40$^{}$ & -0.41$^{}$ & 0.01$^{}$ & -0.05$^{}$ \\ religion$_t$ & -0.25$^{}$ & -0.26$^{}$ & -0.12$^{}$ & -0.22$^{}$ & -0.47$^{*}$ & -0.45$^{}$ & -0.12$^{}$ & -0.04$^{}$ \\ physical$_t$ & -0.63$^{***}$ & -0.62$^{***}$ & -0.52$^{}$ & -0.44$^{}$ & -0.84$^{***}$ & -0.82$^{***}$ & -0.42$^{*}$ & -0.43$^{*}$ \\ search$_t$ & -0.31$^{**}$ & -0.31$^{**}$ & -0.11$^{}$ & -0.18$^{}$ & -0.65$^{***}$ & -0.64$^{***}$ & 0.11$^{}$ & 0.10$^{}$ \\  dine$_t$ & -0.39$^{***}$ & -0.38$^{***}$ & 0.19$^{}$ & 0.19$^{}$ & -0.79$^{***}$ & -0.76$^{***}$ & -0.22$^{}$ & -0.21$^{}$  \\     \bottomrule \\[-1.8ex] Obs. & 552 & 552 & 140 & 140 & 291 & 291 & 121 & 121 \\ $R^2$ & 0.12 & 0.12 & 0.09 & 0.11 & 0.17 & 0.17 & 0.15 & 0.18 \\ Adjusted $R^2$ & 0.10 & 0.10 & -0.00 & 0.01 & 0.14 & 0.13 & 0.06 & 0.08 




\\ \bottomrule
\multicolumn{8}{r}{$^{*}$p$<$0.1; $^{**}$p$<$0.05; $^{***}$p$<$0.01} 

\end{tabular}
\label{trips_car}
\end{table}
\end{center}

==> tables/time_new.tex <==

%\begin{figure}
%\setlength{\fboxsep}{0pt}%
%\setlength{\fboxrule}{0pt}%
%\begin{boxedverbatim}
\begin{landscape}

\begin{table}

\scriptsize\sf\centering
\caption{Effects of $access$ on trip behavior}
\scriptsize
\setlength{\tabcolsep}{4pt}
\begin{tabular}{c | c c | c c c c c c c c c c}
&\multicolumn{2}{c}{A. DV:   $Pr(walk)$ (Poisson)}&\multicolumn{10}{c}{B. DV: $log\;duration$ across various modes (OLS)}\\
\toprule
&&& $all$ & $all$ & $walk$ & $walk$ &$bike$ &$bike$  & $bus$  & $bus$& $auto$ &$auto$
\\
\toprule
\textbf{Ind. Variable} &(A1)&(A2)&(B1) & (B2) & (B3) & (B4) &(B5) &(B6)  &(B7)  & (B8)& (B9) &(B10)\\ 
\midrule
$access(poly)$ && & -0.32***	&-0.16***&&&&&& \\
              && &(0.03)&	(0.05) &&&&&& \\
$access(walk)$ &1.00**&1.00*** &   &      & -0.04***&	-0.02&&&&&&\\
&(0.10)&(0.11)&        & & (0.01)&	(0.02)&&&&&&\\
$access(bike)$  &&&   &      & &&0.22&	0.37&&&&\\
&&&   &      & &&(0.18)&	(0.29)&&&&\\
$access(bus)$  &&&   &      & &&&&-1.02***&	-0.54***&&\\
&&&   &      & &&&&(0.07)&	(0.12)&&\\
$access(auto)$  &-5.66***&-3.60***&   &      & &&&&&&-0.73***	&-0.63***\\
&(0.46)&(0.52) &   &      & &&&&&&(0.13)&	(0.18)\\
$homes(grav)$ &53.83E-8***&15.20E-8** &   5.97E-8***&	2.30E-8**&	2.42E-8***	&0.57E-08	&-1.79E-8&	-6.48E-8&	10.8E-8***&	4.79E-8***&	8.99E-8***&	8.06E-8***\\
&(5.25E-8)&(6.67E-8)&      (0.08E-8)&	(1.03E-8)	&(0.93E-8)	&(1.1E-8)&	(4.99E-8)	&(6.95E-8)	&(1.3E-8)	&(1.6E-8)&	(2.05E-8)&	(2.91E-8)\\
$stratum$  &&-0.31***& &	-0.03***	&&	-0.01*	&&	-0.03	&&	-0.05***	&&0.00\\
&&(0.03)&       &	(0.01)	&&	(0.01)	&&	(0.04)	&&	(0.01)	&&	(0.01)\\
$stratum\times access$ &&0.02 &   &	-0.01***	&&	-0.02***	&&	-0.05&&		-0.01		&&-0.02**\\
&	(0.01)&&(0.02)&   &(0.00)	&&	(0.01)	&&	(0.03)	&&	(0.01)	&\\
$const$&-0.57**&-0.35 & 1.73***&	1.81***	&1.25***	&1.34***	&1.40***	&1.55***	&2.28***&	2.23***	&1.92***	&1.88***\\
  &(0.23)&(0.25)           &  (0.03)&	(0.03)	&(0.04)&	(0.05)	&(0.17)&	(0.20)	&(0.04)&	(0.05)&	(0.07)	&(0.08)\\
Mode FE    &&       &  X &X       &&&&&&&&\\    
Weekday FE &-0.12***&-0.10***& -0.00	&-0.00	&-0.01&	-0.01	&-0.00	&-0.00	&-0.00	&-0.00&	0.03	&0.02\\
Searching FE &2.03***&2.02***& -0.14***	& -0.14***	& -0.24***& 	-0.24***& 	-0.29***& 	-0.30***&-0.03&	-0.03	&-0.21***&	-0.21***\\
Eating FE&2.61***&2.67***&  -0.21***&	-0.20***	&-0.30***	&-0.30***&	-0.22*	&-0.22*&	-0.21***	&-0.19***	&-0.23***	&-0.23***\\
Shopping FE &3.14***&3.15*** &-0.24***&	-0.23***&	-0.33***&	-0.33***&	-0.43***&	-0.43***&	-0.12***&	-0.12***	&-0.28***	&-0.28***\\
Errand FE&1.36***&1.37***&  -0.05***&	-0.05***&	-0.12***&	-0.12***&	-0.21**&	-0.21**&	-0.03***&	-0.03***&	-0.10***&	-0.10***\\
Recreational FE&2.11***&2.13***&  -0.11***&	-0.11***&	-0.19***&	-0.19***&	-0.25**	&-0.26**&	-0.14***&	-0.13***&	-0.11***&	-0.11***\\
Religious FE&2.21***&2.22***&  -0.11***&	-0.11***&	-0.23***&	-0.23***&	-0.21	&-0.21&	-0.05*&	-0.05*&	-0.15***&	-0.15***\\
Physical FE&3.21***&3.26***&  -0.14***&	-0.14***&	-0.23***&	-0.23***&	-0.21***&	-0.21**&	-0.14***&	-0.14***&	-0.27***&	-0.27***\\
Age&0.01***&0.01***&  0.00***&	0.00***	&0.00***&	0.00***	&0.00*	&0.00*	&-0.00**&	-0.00*	&0.00&	0.00\\
Female FE&0.43***&0.43***&  0.00&	0.00&	0.00&	0.00&	-0.02&	-0.02&	-0.01	&-0.01&	0.01&	0.01\\
\midrule
T  (trips)&15133&15133&15133&	15133&7257&	7257&	561&	561	&4748&	4748&	2245	&2245\\
$R^2$       &&   &0.40 &	0.40 &	0.08 &	0.08 &	0.08 &	0.08 &	0.08	 &0.08 &	0.10 &	0.10 \\
Pseudo-$R^2$     &0.20&0.20     & &	 &	 &	&	 &	 &		 & &	 &	 \\
\bottomrule
\end{tabular}

\label{trips_pwalk}
\end{table}
%\end{boxedverbatim}
%\end{center}
%\caption{Example table layout.\label{F2}}
\end{landscape}

==> tables/time_table.tex <==

%\begin{figure}
%\setlength{\fboxsep}{0pt}%
%\setlength{\fboxrule}{0pt}%
\begin{center}
%\begin{boxedverbatim}
\begin{table}

\scriptsize\sf\centering
\caption{Effects of accessibility on trip time}
\textbf{Dep. Variable}: $log \;time_{t,u,i}$ (all modes)\\

\begin{tabular}{c | c c c c c c }
\toprule
\textbf{Ind. Variable} & $trips$ &  & $respondents$ & & $cells$ & \\ 
\midrule
$CA_i(poly)$  & 0.01**  &     0.02***   &   0.01**  &  0.02***   & -0.00** &0.00\\
               & (0.01)  &   (0.01)   &    (0.01) & (0.01)      & (0.01)&(0.01)\\
$stratum_i$     &       &   -0.02***  &           &  -0.01**  & & -0.01***\\
                &       &   (0.01)    &          &   (0.01)  &&(0.01)\\
$Const$       & 1.43***   &   1.46***    1.45*** &   1.48***   & 1.45***&1.47***\\
             &  (0.00)    &  (0.01)    & (0.00)  &    (0.01)   & (0.01)&(0.02)\\ 
        
        \midrule
N     &13748 &  13748 &  12286&  12286 & 119 & 119\\
$R^2$          &0.00  &    0.00      & 0.00  &0.00       & 0.00 &0.14\\

\bottomrule
\end{tabular}
\\

\textbf{Dep. Variable}: $time_{t,u,i}$ (walking)\\

\begin{tabular}{c | c c c c c c }
\toprule
\textbf{Ind. Variable} & $trips$ &  & $respondents$ & & $cells$ & \\ 
\midrule
$CA_i(walk)$  & 0.01&     0.01   &   0.01  &  0.01   & 0.00 &-0.02\\
               & (0.01)  &   (0.01)   &    (0.01) & (1.0)      & (0.01)&(0.01)\\
$stratum_i$     &       &   0.00  &         &  0.01  & & 0.02**\\
                &       &   (0.01)    &          &   (0.01)  &&(0.02)\\
$Const$       & 1.16***   &   1.15***    & 1.16*** &   1.15***   & 1.16***&1.10***\\
             &  (0.01)    &  (0.02)    & (0.01)  &    (0.02)   & (0.01)&(1.03)\\ 
        
        \midrule
N    &6193 &  6193 &  12286&  12286 & 119 & 119\\
$R^2$          &0.00  &    0.00      & 0.00  &0.00       & 0.00 &0.01\\

\bottomrule
\end{tabular}
\\
\textbf{Dep. Variable}: $log\;time_{t,u,i}$ (bike trips)\\

\begin{tabular}{c | c c c c c c }
\toprule
\textbf{Ind. Variable} & $trips$ &  & $respondents$ & & $cells$ & \\ 
\midrule
$CA_i(bike)$  & 0.12***&   0.15***   &   0.12***  & 0.15***   & 0.12*** &0.15***\\
               & (0.02)  &   (0.03)   &    (0.03) & (0.04)      & (0.04)&(0.04)\\
$stratum_i$     &       &   -0.07*  &         &  -0.07*  & & -0.06\\
                &       &   (0.04)    &          &   (0.04)  &&(0.04)\\
$Const$       & 1.39***   &   1.56***& 1.39*** &  1.57***   & 1.40***&1.56***\\
             &  (0.03)    &  (0.01)    & (0.02)  &    (0.10)   & (0.03)&(0.11)\\ 
        
        \midrule
N &459 &  459 & 441&  441 & 101 & 101\\
$R^2$          &0.04  &    0.05      & 0.04  &0.04       & 0.10 &0.12\\

\bottomrule
\end{tabular}
\\
\textbf{Dep. Variable}: $log\;time_{t,u,i}$ (bus trips)\\

\begin{tabular}{c | c c c c c c }
\toprule
\textbf{Ind. Variable} & $trips$ &  & $respondents$ & & $cells$ & \\ 
\midrule
$CA_i(bus)$  & -0.09***&   -0.05***   &   -0.09***  & -0.05***   & -0.09*** &-0.06\\
               & (0.01)  &   (0.01)   &    (0.01) & (0.01)      & (0.01)&(0.02)\\
$stratum_i$     &       &   -0.06***  &         &  -0.06***  & & -0.05***\\
                &       &   (0.01)    &          &   (0.01)  &&(0.01)\\
$Const$       & 1.90***   &   2.06***& 1.90*** &  2.06***   & 1.93***&2.05***\\
             &  (0.01)    &  (0.03)    & (0.01)  &    (0.03)   & (0.01)&(0.04)\\ 
        
        \midrule
N    &1356 &  1356 &  1349&  1349 & 117 & 117\\
$R^2$          &0.07  &    0.09      & 0.07  &0.09       & 0.27 &0.33\\

\bottomrule
\end{tabular}
\\
\textbf{Dep. Variable}: $log \;time_{t,u,i}$ (automobile trips)\\

\begin{tabular}{c | c c c c c c }
\toprule
\textbf{Ind. Variable} & $trips$ &  & $respondents$ & & $cells$ & \\ 
\midrule
$CA_i(auto)$  & -0.05***&   -0.04***   &   -0.06***  & -0.04***   & -0.06*** &-0.02\\
               & (0.01)  &   (0.01)   &    (0.01) & (0.01)      & (0.02)&(0.02)\\
$stratum_i$     &       &   -0.01*  &         &  -0.02**  & & -0.05***\\
                &       &   (0.01)    &          &   (0.01)  &&(0.02)\\
Trip-level controls
$Const$      & 1.55***   &   1.59***& 1.56*** &  1.61***   & 1.59***&1.72***\\
             &  (0.01)    &  (0.02)    & (0.01)  &    (0.03)   & (0.02)&(0.05)\\ 
        
        \midrule
N      &2410 &  2410 &  2278&  2278 & 117 & 117\\
$R^2$          &0.01  &    0.01      & 0.01  &0.01       & 0.08 &0.14\\

\bottomrule
\end{tabular}
\label{table:trips}
\end{table}
%\end{boxedverbatim}
\end{center}
%\caption{Example table layout.\label{F2}}
%\end{figure}

==> tables/walk_propensity.tex <==

%\begin{figure}
%\setlength{\fboxsep}{0pt}%
%\setlength{\fboxrule}{0pt}%
%\begin{center}
%\begin{boxedverbatim}
\begin{table}

\scriptsize\sf\centering
\caption{Effects of accessibility on propensity to make walking trips}
\textbf{Dep. Variables}: Pr($mode_t=walk$) (logistic regression on trips);\\ Pr($|walk \;trips|=k$ for $k=1...|walk\;trips|$) (Poisson regression on respondents);\\ $\% walking \;trips$ (WLS on cells) \\
\begin{tabular}{c | c c c c c c }
\toprule
\textbf{Ind. Variable} & $trips$  & & $respondents$&  & $cells$&  \\ 
\midrule
$CA_i(walk)$  &-0.11***&     0.13***   &   -0.08***  &  0.06**   & -0.03* &0.03**\\
               & (0.02)  &   (0.04)   &    (0.02) & (0.03)      & (0.01)&(0.02)\\
$stratum_i$     &       &   -0.28***  &         &  -0.16***  & & -0.07***\\
                &       &   (0.03)    &          &   (0.02)  &&(0.01)\\
$Const$       & -0.08***   &   0.66***    & -1.83*** &   1.40***   & 0.47***&0.64***\\
             &  (0.02)    &  (0.08)    & (0.02)  &    (0.06)   & (0.01)&(0.03)\\ 
 \midrule
N  &9829 &  9829 & 8826& 8826 & 118& 118\\
Pseudo-$R^2$          &0.00  &    0.01      & 0.00  &0.00       & &\\
$R^2$           &           &               &       &           &0.03 &0.23\\
\bottomrule
\end{tabular}
\label{table:walk}
\end{table}
%\end{boxedverbatim}
%\end{center}
%\caption{Example table layout.\label{F2}}
%\end{figure}

